Natural Logic-guided Autoregressive Multi-hop Document Retrieval for Fact Verification

A key component of fact verification is thevevidence retrieval, often from multiple documents. Recent approaches use dense representations and condition the retrieval of each document on the previously retrieved ones. The latter step is performed over all the documents in the collection, requiring storing their dense representations in an index, thus incurring a high memory footprint. An alternative paradigm is retrieve-and-rerank, where documents are retrieved using methods such as BM25, their sentences are reranked, and further documents are retrieved conditioned on these sentences, reducing the memory requirements. However, such approaches can be brittle as they rely on heuristics and assume hyperlinks between documents. We propose a novel retrieve-and-rerank method for multi-hop retrieval, that consists of a retriever that jointly scores documents in the knowledge source and sentences from previously retrieved documents using an autoregressive formulation and is guided by a proof system based on natural logic that dynamically terminates the retrieval process if the evidence is deemed sufficient. This method is competitive with current state-of-the-art methods on FEVER, HoVer and FEVEROUS-S, while using $5$ to $10$ times less memory than competing systems. Evaluation on an adversarial dataset indicates improved stability of our approach compared to commonly deployed threshold-based methods. Finally, the proof system helps humans predict model decisions correctly more often than using the evidence alone.

==> images/outdated_fig_tikz.tex <==
%\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt      
\begin {figure*}%[!hbtp]
\begin{adjustbox}{width=\textwidth}









\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,328); %set diagram left start at 0, and has height of 328

%Shape: Rectangle [id:dp4189748247920939] 
\draw  [fill={rgb, 255:red, 233; green, 227; blue, 227 }  ,fill opacity=1 ] (4.86,29.57) -- (197.43,29.57) -- (197.43,274.57) -- (4.86,274.57) -- cycle ;
%Flowchart: Process [id:dp7021425489665507] 
\draw   (9.11,50.91) -- (193.43,50.91) -- (193.43,101.97) -- (9.11,101.97) -- cycle ;
%Shape: Rectangle [id:dp19937224770277884] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.71 ] (4,2) -- (416.86,2) -- (416.86,26) -- (4,26) -- cycle ;
%Shape: Rectangle [id:dp5717124553600541] 
\draw  [fill={rgb, 255:red, 186; green, 135; blue, 228 }  ,fill opacity=1 ] (33.43,36.57) -- (156.49,36.57) -- (156.49,54.57) -- (33.43,54.57) -- cycle ;
%Flowchart: Process [id:dp5577876487423852] 
\draw   (9.11,123.9) -- (192.43,123.9) -- (192.43,184.31) -- (9.11,184.31) -- cycle ;
%Shape: Rectangle [id:dp8349880736875497] 
\draw  [fill={rgb, 255:red, 135; green, 188; blue, 228 }  ,fill opacity=1 ] (32.26,107.96) -- (155.32,107.96) -- (155.32,127.57) -- (32.26,127.57) -- cycle ;
%Flowchart: Process [id:dp9729539016345317] 
\draw   (9.94,205.29) -- (193.43,205.29) -- (193.43,265.7) -- (9.94,265.7) -- cycle ;
%Shape: Rectangle [id:dp2213645068409411] 
\draw  [fill={rgb, 255:red, 231; green, 177; blue, 72 }  ,fill opacity=1 ] (33.08,191.57) -- (156.15,191.57) -- (156.15,209.57) -- (33.08,209.57) -- cycle ;
%Flowchart: Alternative Process [id:dp06192404751995806] 
\draw   (215,90.47) .. controls (215,84.14) and (220.14,79) .. (226.47,79) -- (321.38,79) .. controls (327.72,79) and (332.86,84.14) .. (332.86,90.47) -- (332.86,133.1) .. controls (332.86,139.43) and (327.72,144.57) .. (321.38,144.57) -- (226.47,144.57) .. controls (220.14,144.57) and (215,139.43) .. (215,133.1) -- cycle ;
%Flowchart: Process [id:dp1752381291516567] 
\draw  [fill={rgb, 255:red, 231; green, 177; blue, 72 }  ,fill opacity=1 ] (337,156) -- (451.43,156) -- (451.43,176.57) -- (337,176.57) -- cycle ;
%Flowchart: Process [id:dp4834195688063214] 
\draw  [fill={rgb, 255:red, 185; green, 132; blue, 230 }  ,fill opacity=1 ] (340,60.86) -- (450.43,60.86) -- (450.43,78.71) -- (340,78.71) -- cycle ;
%Flowchart: Process [id:dp3652552517753913] 
\draw  [fill={rgb, 255:red, 231; green, 177; blue, 72 }  ,fill opacity=1 ] (341,34.86) -- (448.43,34.86) -- (448.43,54.57) -- (341,54.57) -- cycle ;
%Flowchart: Process [id:dp5781735407268627] 
\draw  [fill={rgb, 255:red, 231; green, 177; blue, 72 }  ,fill opacity=1 ] (339,209.14) -- (451.43,209.14) -- (451.43,226.71) -- (339,226.71) -- cycle ;
%Flowchart: Process [id:dp3744079643333147] 
\draw  [fill={rgb, 255:red, 185; green, 132; blue, 230 }  ,fill opacity=1 ] (337,183.14) -- (451.43,183.14) -- (451.43,201.14) -- (337,201.14) -- cycle ;
%Flowchart: Alternative Process [id:dp9538270528197692] 
\draw   (220.14,245.91) .. controls (220.14,239.12) and (225.65,233.62) .. (232.43,233.62) -- (330.14,233.62) .. controls (336.93,233.62) and (342.43,239.12) .. (342.43,245.91) -- (342.43,291.57) .. controls (342.43,298.35) and (336.93,303.86) .. (330.14,303.86) -- (232.43,303.86) .. controls (225.65,303.86) and (220.14,298.35) .. (220.14,291.57) -- cycle ;
%Straight Lines [id:da6538338995681274] 
\draw [line width=1.5]    (200.86,171.57) -- (265.25,232.79) ;
\draw [shift={(267.43,234.86)}, rotate = 223.55] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da4297031795700803] 
\draw [line width=1.5]    (200.86,171.57) -- (267.61,146.9) ;
\draw [shift={(270.43,145.86)}, rotate = 159.72] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Triangle [id:dp7647990090855719] 
\draw   (500,94.57) -- (535,134.57) -- (465,134.57) -- cycle ;
%Flowchart: Process [id:dp3298515503812287] 
\draw  [fill={rgb, 255:red, 231; green, 177; blue, 72 }  ,fill opacity=1 ] (544,60) -- (654.43,60) -- (654.43,80.57) -- (544,80.57) -- cycle ;
%Flowchart: Process [id:dp11592886605155939] 
\draw  [fill={rgb, 255:red, 231; green, 177; blue, 72 }  ,fill opacity=1 ] (544,89) -- (655.43,89) -- (655.43,109.57) -- (544,109.57) -- cycle ;
%Flowchart: Process [id:dp5657614231295651] 
\draw  [fill={rgb, 255:red, 185; green, 132; blue, 230 }  ,fill opacity=1 ] (543,116.57) -- (655.43,116.57) -- (655.43,134.14) -- (543,134.14) -- cycle ;
%Flowchart: Process [id:dp9736039585330523] 
\draw  [fill={rgb, 255:red, 185; green, 132; blue, 230 }  ,fill opacity=1 ] (543,141.57) -- (655.43,141.57) -- (655.43,161.14) -- (543,161.14) -- cycle ;
%Flowchart: Process [id:dp316015422281392] 
\draw  [fill={rgb, 255:red, 231; green, 177; blue, 72 }  ,fill opacity=1 ] (543,165.14) -- (655.43,165.14) -- (655.43,185.71) -- (543,185.71) -- cycle ;
%Straight Lines [id:da08059072850340998] 
\draw [line width=1.5]    (570,189) -- (570.43,269.57) ;
%Curve Lines [id:da40617336797277637] 
\draw [line width=1.5]    (102.14,279.64) .. controls (258.94,346.61) and (530.83,299.27) .. (570.43,269.57) ;
\draw [shift={(97.43,277.57)}, rotate = 24.17] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Flowchart: Alternative Process [id:dp2701641250751543] 
\draw  [fill={rgb, 255:red, 220; green, 216; blue, 118 }  ,fill opacity=1 ] (455,283) .. controls (455,279.13) and (458.13,276) .. (462,276) -- (527.43,276) .. controls (531.29,276) and (534.43,279.13) .. (534.43,283) -- (534.43,309) .. controls (534.43,312.87) and (531.29,316) .. (527.43,316) -- (462,316) .. controls (458.13,316) and (455,312.87) .. (455,309) -- cycle ;
%Flowchart: Connector [id:dp12653681037508036] 
\draw  [fill={rgb, 255:red, 83; green, 184; blue, 101 }  ,fill opacity=1 ] (7,40.07) .. controls (7,34.27) and (12.24,29.57) .. (18.71,29.57) .. controls (25.18,29.57) and (30.43,34.27) .. (30.43,40.07) .. controls (30.43,45.87) and (25.18,50.57) .. (18.71,50.57) .. controls (12.24,50.57) and (7,45.87) .. (7,40.07) -- cycle ;
%Flowchart: Connector [id:dp3557038565423436] 
\draw  [fill={rgb, 255:red, 83; green, 184; blue, 101 }  ,fill opacity=1 ] (212.24,79.07) .. controls (212.24,73.27) and (217.48,68.57) .. (223.95,68.57) .. controls (230.42,68.57) and (235.66,73.27) .. (235.66,79.07) .. controls (235.66,84.87) and (230.42,89.57) .. (223.95,89.57) .. controls (217.48,89.57) and (212.24,84.87) .. (212.24,79.07) -- cycle ;
%Flowchart: Connector [id:dp5177510779070058] 
\draw  [fill={rgb, 255:red, 83; green, 184; blue, 101 }  ,fill opacity=1 ] (475.24,101.07) .. controls (475.24,95.27) and (480.48,90.57) .. (486.95,90.57) .. controls (493.42,90.57) and (498.66,95.27) .. (498.66,101.07) .. controls (498.66,106.87) and (493.42,111.57) .. (486.95,111.57) .. controls (480.48,111.57) and (475.24,106.87) .. (475.24,101.07) -- cycle ;
%Flowchart: Connector [id:dp8964610080150441] 
\draw  [fill={rgb, 255:red, 83; green, 184; blue, 101 }  ,fill opacity=1 ] (450.29,276) .. controls (450.29,270.2) and (455.53,265.5) .. (462,265.5) .. controls (468.47,265.5) and (473.71,270.2) .. (473.71,276) .. controls (473.71,281.8) and (468.47,286.5) .. (462,286.5) .. controls (455.53,286.5) and (450.29,281.8) .. (450.29,276) -- cycle ;
%Flowchart: Connector [id:dp9192432885128152] 
\draw  [fill={rgb, 255:red, 83; green, 184; blue, 101 }  ,fill opacity=1 ] (214.24,238.07) .. controls (214.24,232.27) and (219.48,227.57) .. (225.95,227.57) .. controls (232.42,227.57) and (237.66,232.27) .. (237.66,238.07) .. controls (237.66,243.87) and (232.42,248.57) .. (225.95,248.57) .. controls (219.48,248.57) and (214.24,243.87) .. (214.24,238.07) -- cycle ;

% Text Node
\draw (4,2) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize C: The United States dollar is used in terrirory owned by the United Kingdom}};
% Text Node
\draw (9.11,50.91) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize The dollar coin is a United States coin}\\{\scriptsize  worth one United States dollar.}};
% Text Node
\draw (9.11,123.9) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize The United Kingdom of Great Britain}\\{\scriptsize  and Northern Ireland , commonly}\\{\scriptsize  known as the United Kingdom (UK) ... }};
% Text Node
\draw (30.43,40.07) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Dollar coin (US)}};
% Text Node
\draw (7.81,108.59) node [anchor=north west][inner sep=0.75pt]   [align=left] {};
% Text Node
\draw (32.26,107.96) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{60.78pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize United Kingdom}
\end{center}

\end{minipage}};
% Text Node
\draw (9.94,205.29) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Besides the United States , it is used}\\{\scriptsize as the sole currency in two \underline{\textbf{British}}}\\{\scriptsize \underline{\textbf{Overseas Territories}} in the Caribbean.}};
% Text Node
\draw (33.08,191.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{73.94pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize United States dollar}
\end{center}

\end{minipage}};
% Text Node
\draw (216,90.47) node [anchor=north west][inner sep=0.75pt]   [align=left] {Autoregressive\\Query Generator};
% Text Node
\draw (341,34.86) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize United States Dollar}};
% Text Node
\draw (337,156) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \underline{\textbf{British Overseas ...}}}};
% Text Node
\draw (337,183.14) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize United States}};
% Text Node
\draw (339,209.14) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Carribean}};
% Text Node
\draw (340,60.86) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Dollar coin (US)}};
% Text Node
\draw (226.14,242.09) node [anchor=north west][inner sep=0.75pt]   [align=left] {Natural Logic\\Sufficency Proof\\ Generator};
% Text Node
\draw (461,43) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Merge of}\\{\footnotesize  $\displaystyle D_{t}{}_{-1}$ and $\displaystyle \overline{D_{t}}$}};
% Text Node
\draw (156.15,27.84) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle E_{t}{}_{- 1}$};
% Text Node
\draw (574,206) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle D_{t}$};
% Text Node
\draw (478,109) node [anchor=north west][inner sep=0.75pt]   [align=left] {Proof};
% Text Node
\draw (544,60) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize United States Dollar}};
% Text Node
\draw (544,89) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \underline{\textbf{British Overseas...}}}};
% Text Node
\draw (543,116.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Dollar coin (US)}};
% Text Node
\draw (543,141.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize United States}};
% Text Node
\draw (543,165.14) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Carribean}};
% Text Node
\draw (462,286.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {Reranker};
% Text Node
\draw (404,284) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle E_{t}$};
% Text Node
\draw (11.76,28.72) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (219,226.72) node [anchor=north west][inner sep=0.75pt]   [align=left] {3};
% Text Node
\draw (217,67.72) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (480,86.72) node [anchor=north west][inner sep=0.75pt]   [align=left] {4};
% Text Node
\draw (454,264.72) node [anchor=north west][inner sep=0.75pt]   [align=left] {5};
% Connection
\draw [line width=1.5]    (336,90.41) -- (348.41,85.89) ;
\draw [shift={(351.23,84.86)}, rotate = 159.96] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
% Connection
\draw [line width=1.5]    (325.24,135.47) -- (364.74,153.74) ;
\draw [shift={(367.47,155)}, rotate = 204.82] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
% Connection
\draw [line width=1.5]    (342.14,274.4) .. controls (452.17,282.37) and (504.59,235.74) .. (499.43,134.53) ;
\draw [shift={(499.35,133)}, rotate = 86.77] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
% Connection
\draw [line width=1.5]    (414.97,84.86) -- (474.24,110) ;
\draw [shift={(477,111.17)}, rotate = 202.99] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
% Connection
\draw [line width=1.5]    (422.29,155) -- (474.26,131.63) ;
\draw [shift={(477,130.39)}, rotate = 155.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

\end{tikzpicture}

\end{adjustbox}
\end{figure*}
